Post hoc Explanations may be Ineffective for Detecting Unknown Spurious Correlation

We investigate whether three types of post hoc model explanations--feature attribution, concept activation, and training point ranking--are effective for detecting a model's reliance on spurious signals in the training data. Specifically, we consider the scenario where the spurious signal to be detected is unknown, at test-time, to the user of the explanation method. We design an empirical methodology that uses semi-synthetic datasets along with pre-specified spurious artifacts to obtain models that verifiably rely on these spurious training signals. We then provide a suite of metrics that assess an explanation method's reliability for spurious signal detection under various conditions. We find that the post hoc explanation methods tested are ineffective when the spurious artifact is unknown at test-time especially for non-visible artifacts like a background blur. Further, we find that feature attribution methods are susceptible to erroneously indicating dependence on spurious signals even when the model being explained does not rely on spurious artifacts. This finding casts doubt on the utility of these approaches, in the hands of a practitioner, for detecting a model's reliance on spurious signals.

==> datatable.tex <==


\begin{table*}[t]
\centering
\rowcolors{1}{}{lightgray}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{llllc}
\hline
%\multicolumn{2}{c}{Item} \\
%\cline{1-2}
\textbf{Task}   & \textbf{Input Data} & \textbf{Categories} & \textbf{Model} & \textbf{Accuracy Metrics} \\
\hline
Bone Age Classification & Bone Image & Categories & ResNet-50 & blah \\

Knee Arthritis Classification & Bone Image & Categories & ResNet-50 & blah \\

Bird Species Classification & Bone Image & Categories & ResNet-50 & blah \\
\end{tabular}
}
\caption{Example bugs we test for each bug categories and their formalization.}
\label{tab:bugformalization_main}
\end{table*}

==> results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% normal model section
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Insights into the `Normal' Model.\myworries{The exact way to structure this section is not clear in my mind, so will iterate.}}
\label{sec:normal}
\begin{wrapfigure}{r}{0.25\textwidth}
\begin{center}
\includegraphics[scale=0.25]{figures/spurious_bug_easy_demo.png}
 \end{center}
\caption{\textbf{Spurious Hospital Tag on Training Image.}}
\label{fig:spuriouseasydemo}
\end{wrapfigure}
We now discuss the insights that can be gleaned a normally trained model. Due to space limitations, we describe results for the feature attribution methods here and defer discussion on training point ranking and concept attribution to the appendix. Overall, we find that each of the $3$ methods provides insights that suggest that the normal model is reliable. In the next section, we will contrast the insights discussed in this section with those gleaned from a model that has been spurious to manifest spurious signals.

\paragraph{Feature Attribution Methods.} In Figure~\ref{fig:array}-A we show $4$ feature attributions for $5$ different inputs (one per each class) for a the normal model. We observe that Gradient, SmoothGrad, and Integrated Gradients seem to highlight relevant parts of the input that a radiologist might pay attentions to. In the case of Guided Backprop, we observe that the feature attributions seem to approximate the input, which confirms insights from previous work~\citep{nie2018theoretical}. 

%%%%%%%%%%%%%%%%%%%%%%%%
%spurious correlation
%%%%%%%%%%%%%%%%%%%
\section{Detecting Spurious Correlation.}
\label{sec:spurious}
In this section, we explain models that have been induced to rely on spurious training set signals. We show that unless one knows to test for these spurious signals explicitly, detecting that the model relies on a spurious signal for classification is challenging with the $3$ explanation methods that we consider. We demonstrate this difficulty both for an `easy' spatial spurious signal and a challenging, non-obvious signal as well.

% Figure showing the supervised ML pipeline and bugs at each stage of that pipeline.
\begin{figure*}[h]
\centering
\includegraphics[scale=0.400]{figures/attribution_spurious_demo.png}
\caption{Feature Attribution Spurious Correlation Results. A: we show attributions for all methods on a spurious model, but these inputs do not have the hospital tag, which is the spurious signal. B: We show attributions for all methods on a spurious model, but these inputs have the hospital tag.}
\label{fig:attributionspurious}
\end{figure*}

% Figure showing the supervised ML pipeline and bugs at each stage of that pipeline.
\begin{figure*}[h]
\centering
\includegraphics[scale=0.35]{figures/tcav_spurious_correlation_results.png}
\caption{TCAV Spurious Correlation Results. In A, we show the TCAV rankings for a the easy spurious model setting, and B we show the TCAV rankings for the hard spurious setting. In column 6, we show the concept ranking where we have explicitly tested for the model's dependence on the spurious signal.}
\label{fig:tcavspurious}
\end{figure*}

\begin{figure*}[!h]
\centering
\includegraphics[scale=0.35]{figures/influence_functions_spurious_correlation_results.png}
\caption{Influence Functions Spurious Correlation Results for the easy setting. In the first two columns, we show present the metric: for a given test-input, what is the fraction of the top $20$ ranked training inputs that belong to the true class of the test-input--across all classes for the normal model and the spurious model. On the far right, we should an example for a test-input that includes the spurious hospital signal.}
\label{fig:influencespurious}
\end{figure*}

\paragraph{Experimental Setting.} Spurious training signals are artifacts that encode and correlate with the input label in the training set but are not meaningfully useful for generalization. Here we consider two spurious signals as spurious signals. In the first case, which constitutes the easy settings, we `paste' a hospital code (in this MGH for a hypothetical hospital) onto the images for all inputs for the class Pre-Puberty. See Figure~\ref{fig:spuriouseasydemo} for an example. Here, the model trained on this task is than forced to use the spurious hospital code as a `short-cut' for the Pre-Puberty class.

In the second spurious setting, we use a low frequency grid noise pattern that is not visible to the eye as the spurious training signal. We can selectively add this patterned noise to inputs in a specific class stochastically. We empirically verify that a model trained on this modified dataset learns to use the patterned noise as a short-cut. We now discuss whether the post hoc interpretations considered are able to signal that the model relies on this spurious signal.

\paragraph{Feature Attribution.} We derive feature attributions for $5$ different test inputs, one per class, for the $4$ feature attribution methods tested for the easy (hospital tag) setting. In general, for both settings, we make similar observations. 

In Figure~\ref{fig:attributionspurious}~we show attributions for all methods on a spurious model, but for inputs that do not have the hospital tag, which is the spurious signal. We observe that the attributions obtained for this setting is qualitatively and quantitatively different from those obtained from a the normal model except in the case of Guided Backpropagation. We observe dispersed attribution across the input, but no clear signal exists to indicate that the model relies on a short-cut. If one only examines the validation and test-set metrics, we actually find that the spurious model performs within $3$ percent of the test accuracy of the normal model. Yet observing Figure~\ref{fig:attributionspurious}-A, one is left with an inconclusive diagnosis.

However, we compute feature attributions again, but for test images where we have artificially inserted the spurious hospital tag. Immediately, as shown in Figure~\ref{fig:attributionspurious}-B, we observe that the attributions focus on the tag. To confirm the reliability of these methods, we quantitatively compare these attributions to ground-truth equivalents and observe similarity (SSIM) greater than $0.78$ across all methods. The situation above demonstrates that unless one explicitly tests for a specific spurious correlation, it is unlikely to be identified by naive feature attribution inspection.

==> testtable.tex <==
\begin{table} % Add the following just after the closing bracket on this line to specify a position for the table on the page: [h], [t], [b] or [p] - these mean: here, top, bottom and on a separate page, respectively
\centering % Centres the table on the page, comment out to left-justify
\begin{tabular}{l c c c c c} % The final bracket specifies the number of columns in the table along with left and right borders which are specified using vertical pipes (|); each column can be left, right or center-justified using l, r or c. Columns will widen to hold the content in them by default, to specify a precise width, use p{width}, e.g. p{5cm}
\toprule % Top horizontal line
& \multicolumn{5}{c}{\textbf{Growth Media}} \\ % Amalgamating several columns into one cell is done using the \multicolumn command with the number of columns to amalgamate as the first argument and then the justification (l, r or c)
\cmidrule(l){2-6} % Horizontal line spanning less than the full width of the table - you can add (r) or (l) just before the opening curly bracket to shorten the rule on the left or right side
\textbf{Strain} & 1 & 2 & 3 & 4 & 5\\ % Column names row
\midrule % In-table horizontal line
GDS1002 & 0.962 & 0.821 & 0.356 & 0.682 & 0.801\\ % Content row 1
NWN652 & 0.981 & 0.891 & 0.527 & 0.574 & 0.984\\ % Content row 2
PPD234 & 0.915 & 0.936 & 0.491 & 0.276 & 0.965\\ % Content row 3
JSB126 & 0.828 & 0.827 & 0.528 & 0.518 & 0.926\\ % Content row 4
JSB724 & 0.916 & 0.933 & 0.482 & 0.644 & 0.937\\ % Content row 5
\midrule % In-table horizontal line
\midrule % In-table horizontal line
Average Rate & 0.920 & 0.882 & 0.477 & 0.539 & 0.923\\ % Summary/total row
\bottomrule % Bottom horizontal line
\end{tabular}
\caption{Table caption text} % Table caption, can be commented out if no caption is required
\label{tab:template} % A label for referencing this table elsewhere, references are used in text as \ref{label}
\end{table}
